Can Vision-Language-Action Models Learn from Real-World Data Continually without Forgetting?

Vision-Language-Action (VLA) models provide a promising foundation for general-purpose robotics, yet their real-world deployment demands the ability to continually acquire new skills without forgetting prior ones. While recent studies have explored continual learning for VLA models in simulated settings, the challenge remains largely unexamined under realistic physical conditions. To bridge this gap, we construct a real-world continual learning benchmark comprising ten diverse sequential manipulation tasks across both single-arm and bimanual configurations. Through extensive experiments on this benchmark, we find that naive sequential fine-tuning leads to severe catastrophic forgetting, whereas a well-configured experience replay (ER) approach can effectively mitigate forgetting and outperform joint multi-task training under equivalent computational budgets. Notably, by synthesizing our empirical findings, we successfully achieve stable continual learning across the full 10-task heterogeneous stream, retaining previously acquired capabilities while adapting to diverse new skills in real-world deployment. This work presents an empirical study grounded in real-world continual VLA learning and offers actionable insights for deploying robust, long-lived robotic policies.

==> main.tex <==
\section{Introduction}

Vision-Language-Action (VLA) models have emerged as a promising paradigm for general-purpose robotics by unifying visual perception, language understanding, and action generation within a single policy \cite{ma2024survey,kim2025openvla}. Pretrained on large-scale robotic datasets, these models exhibit impressive cross-task generalization and transfer capabilities for embodied control \cite{black2025pi}. However, practical deployment demands capabilities beyond static, single-stage performance, where robots must continually acquire new skills from non-stationary data streams without degrading previously learned abilities. This requirement is closely related to catastrophic forgetting, a significant challenge in continual learning, in which sequential model updates unintentionally erase prior knowledge \cite{de2021continual,wang2024comprehensive}. While naively updating VLA models on new task streams causes severe skill degradation, periodically retraining them from scratch on the entire accumulated dataset is computationally prohibitive. Consequently, developing effective mechanisms to mitigate catastrophic forgetting is essential for scalable and lifelong robot learning.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/preface.pdf}
    \caption{This paper investigates continual adaptation of VLA models under real-world robotic data streams. Our ER-based approach achieves robust continual learning performance across diverse manipulation tasks.}
    \label{fig:placeholder}
\end{figure}

% Second, let's write the second paragraph of the Introduction. We need to introduce the current pioneering work of continual learning in VLA models. Read these references and summarize each with 1-2 sentences before merging them smoothly. Then, highlight that VLA models that learn from real-world data continually remain underexplored.
Recent studies have begun to explore continual learning in VLA models from various perspectives. For example, \cite{liu2026pretrained} shows that large pretrained VLAs exhibit notable inherent resistance to forgetting, where model scale, pretraining priors, and even minimal replay buffers significantly enhance skill retention during sequential updates. Furthermore, \cite{hu2026simple} demonstrates that simple sequential fine-tuning combining pretrained VLAs, parameter-efficient adaptation, and on-policy reinforcement learning can overcome catastrophic forgetting while maintaining a favorable balance among retention, plasticity, and generalization. To address settings where historical data is constrained or unavailable, \cite{romer2026clare} proposes a dynamic adapter expansion framework that freezes existing model parameters and fine-tunes dedicated task-specific adapters to prevent parameter overwriting. Meanwhile, \cite{liu2026towards} explores reinforcement fine-tuning tailored for long-lived robots, using on-policy interactions to enable continuous adaptation of VLA models while avoiding the severe skill degradation common in standard supervised fine-tuning.


Despite these advances, existing continual learning evaluations for VLA models suffer from key limitations that systematically overestimate their robustness to forgetting. \textbf{First, simulation-based benchmarks lack the heterogeneity found in physical deployments.} Dominant benchmarks such as LIBERO \cite{liu2023libero} evaluate narrowly defined subtasks under fixed embodiments, environments, and action spaces. Such limited distribution shifts tend to underestimate forgetting, as retaining performance across highly correlated tasks does not guarantee generalization to heterogeneous real-world deployments. \textbf{Second, the observed resistance to forgetting may be confounded by overlap with pretraining data.} As noted by \cite{liu2026pretrained}, performance retention during sequential updates often stems from pretraining priors rather than algorithmic efficacy. Since standard benchmarks are frequently included in VLA pretraining corpora, high retention scores may simply reflect the reactivation of memorized skills rather than effective continual learning. \textbf{Third, standard evaluation protocols frequently violate causality.} These studies \cite{liu2026pretrained,hu2026simple} precompute global statistics (\eg, action normalization parameters) across the entire task stream before sequential training, thereby leaking future information into the learning process. Reported success is thus an artifact of an unrealistic, information-privileged regime unavailable in real-world deployment. These issues raise questions about whether current findings generalize to realistic settings and obscure whether forgetting in VLA models stems primarily from algorithmic failure or from overlooked factors, such as distributional inconsistency, normalization drift, and optimization imbalance under real-world sequential data.

Inspired by the discussions above, we shift the evaluation of continual learning in VLA models from simulation to physical environments under realistic deployment constraints. Our main contributions are threefold: 

\begin{itemize}
    \item We establish a real-world continual manipulation benchmark comprising ten sequential manipulation tasks (5 single-arm + 5 bimanual) characterized by high task diversity, including rigid-object pick-and-place, contact-rich pressing, and deformable-object folding, etc. To support standardized research, we collect 4,000 high-quality demonstration trajectories and commit to fully open-sourcing the benchmark suite, dataset, and codebase. 

    \item We systematically investigate the key factors governing real-world VLA adaptation, showing first that naive sequential supervised fine-tuning leads to severe catastrophic forgetting on real-world demonstration data streams. Then, we evaluate the experience replay-based approach, demonstrating that its performance significantly depends on proper configurations and highlighting the crucial role of action normalization strategies in maintaining stability during continual learning. 

    \item We successfully achieve robust continual learning across a 10-task heterogeneous real-world manipulation task stream. By synthesizing our empirical findings into a well-configured experience replay and action normalization pipeline, our approach effectively retains past capabilities while acquiring diverse skills, outperforming joint multi-task training under equivalent compute budgets in real-world deployment scenarios.
\end{itemize}

\section{Related Work}
VLA models extend vision-language backbones to physical manipulation by mapping multimodal inputs to actions, with recent advances ranging from autoregressive tokenization~\cite{kim2024openvla} to flow-matching policies~\cite{black2024pi_0,black2025pi}, as well as explorations in diffusion-based policies~\cite{liu2025rdt}, cross-embodiment datasets~\cite{zheng2026xvla}, and post-training paradigms~\cite{llava-vla,sun2026atomvla}. Despite these progresses, current VLAs are predominantly evaluated on fixed datasets rather than non-stationary task streams. Meanwhile, continual learning has established various strategies to mitigate catastrophic forgetting under shifting data distributions~\cite{de2021continual,wang2024comprehensive}, including regularization-based methods \cite{serra2018overcoming,schwarz2018progress,ritter2018online}, architecture-based methods \cite{rusu2016progressive,mallya2018packnet,fernando2017pathnet}, optimization-based methods \cite{lopez2017gradient,chaudhry2018efficient,tang2021layerwise}, and replay-based methods \cite{rebuffi2017icarl,rolnick2019experience,buzzega2020dark}. Among these, experience replay (ER) is widely adopted for its simplicity and effectiveness in preserving historical knowledge~\cite{rolnick2019experience,buzzega2020dark}. While recent studies have explored VLA continual learning in simulation~\cite{liu2026pretrained,hu2026simple}, our work shifts to real-world physical robot data streams, where we find that naive sequential fine-tuning induces significantly more severe forgetting, and that effective adaptation critically depends on proper replay configurations and consistent action normalization.


% \paragraph{Vision-Language-Action Models}
% VLA models extend vision-language backbones to physical manipulation by directly mapping multimodal inputs to executable action spaces. Early VLA architectures primarily employ autoregressive action tokenization, as exemplified by models such as OpenVLA~\cite{kim2024openvla}. More recent foundational policies, such as $\pi_0$~\cite{black2024pi_0} and $\pi_{0.5}$~\cite{black2025pi}, introduce continuous flow-matching heads to capture complex multimodal action distributions at high control frequencies. Alongside architectural scaling, recent research has explored diverse dimensions of policy learning, including diffusion-based manipulation policies~\cite{liu2025rdt}, cross-embodiment datasets~\cite{zheng2026xvla}, action-centric world modeling~\cite{worldvla}, and scalable post-training or reinforcement learning paradigms~\cite{llava-vla,sun2026atomvla}. Despite these advances in static multi-task pretraining and offline fine-tuning, current VLA frameworks are predominantly evaluated on fixed datasets instead of non-stationary task streams. In contrast to standard post-training protocols, our work focuses on the continual adaptation of VLAs under sequential, heterogeneous real-world data, systematically investigating the factors governing physical skill retention and policy stability.

\begin{figure*}[t!]
\centering
\includegraphics[width=\linewidth]{figures/robot_setup.pdf}
\caption{
Overview of the robot platform, individual manipulation tasks, stepwise evaluation protocol, and two distinct continual task streams. These tasks span rigid-body manipulation, bimanual coordination, and complex deformable-object manipulation, requiring diverse motion primitives and providing a comprehensive benchmark for evaluating the continual learning capability of VLA models in real-world scenarios.} 
\label{fig:robot_setup}
\end{figure*}

% \paragraph{Continual Learning}
%  Continual learning studies how agents acquire new capabilities sequentially while mitigating catastrophic forgetting under non-stationary data distributions \cite{de2021continual,wang2024comprehensive,shi2025continual}. Predominant paradigms of continual learning approaches include regularization-based methods \cite{serra2018overcoming,schwarz2018progress,ritter2018online}, architecture-based methods \cite{rusu2016progressive,mallya2018packnet,fernando2017pathnet}, optimization-based methods \cite{lopez2017gradient,chaudhry2018efficient,tang2021layerwise}, and replay-based methods \cite{rebuffi2017icarl,rolnick2019experience,buzzega2020dark}. Among these, experience replay is a widely used strategy that eliminates forgetting by storing and interleaving historical samples during sequential optimization. While pioneering works~\cite{liu2026pretrained,hu2026simple} evaluate VLA continual learning on simulated benchmarks, we focus on real-world adaptation using physical robot demonstration streams. In contrast to simulation, real-world sequential fine-tuning induces severe catastrophic forgetting. We show that policy stability under physical deployment constraints relies heavily on execution-level choices, specifically proper ER configurations and consistent action normalization strategies.

\section{Preliminaries}
\paragraph{Continual Robot Learning.}
We model the robot learning problem as a finite-horizon Markov decision process \cite{puterman1990markov}, defined by the tuple $\mathcal{M}=(\mathcal{S}, \mathcal{A}, \mathcal{T}, H, \mu_0, R)$. Here, $\mathcal{S}$ is the state space, $\mathcal{A}$ is the action space, $\mathcal{T}:\mathcal{S}\times\mathcal{A}\rightarrow\mathcal{S}$ is the transition function, $H$ is the finite episode horizon, $\mu_0$ is the initial state distribution, and $R:\mathcal{S}\times\mathcal{A}\rightarrow\mathbb{R}$ is the reward function. To evaluate the task success, we assume a sparse-reward setting and replace $R$ with a binary goal indicator $g:\mathcal{S}\rightarrow\{0,1\}$. Finally, the goal of the robot is to learn a policy $\pi$ that maximizes the expected return $J_{\rm RL}^\pi=\mathbb{E}_{(\bm{s}_t,\bm{a}_t)\sim\pi,\mu_0}\left[\sum_{t=1}^{H}g(\bm{s}_t)\right]$.

In the continual robot learning scenario, the robot learns a sequence of tasks $\{T^{k}\}_{k=1}^{K}$ with a single policy $\pi(\cdot|\bm{s};T)$ that conditions on the task. Notably, each task $T^k$ is defined by a unique initial state distribution $\mu_0^k$ and a goal predicate $g^k$, while all the tasks share the same $(\mathcal{S},\mathcal{A},\mathcal{T},H)$. Upon receiving the $k$-th task, the robot aims to maximize 
\begin{equation}
    J_{\rm CRL}^\pi=\frac{1}{k}\sum_{p=1}^{k}\left[\mathbb{E}_{(\bm{s}_t^p,\bm{a}_t^p)\sim \pi(\cdot;T^p),\mu^p_0}\left[ \sum_{t=1}^{H}g^{p}(\bm{s}_t^{p})\right]\right].
\end{equation}

\paragraph{Continual Imitation Learning.}
In this paper, we focus on the continual robot learning via imitation learning, especially the supervised fine-tuning (FT) of VLA models. Given expert demonstrations $\mathcal{D}^k=\{\tau_i^k\}_{i=1}^N$ for each task $T^{k}$, where each trajectory $\tau=\{(\bm{o}_{0},\bm{a}_0),\dots,(\bm{o}_{l^k},\bm{a}_{l^k})\},l^k\leq H$ consists of robot sensory inputs $\bm{o}_t$ and actions $\bm{a}_t$. Upon receiving the $k$-th task, our objective is to learn a policy that minimizes:
\begin{equation}
    J_{\rm BC}^\pi=\frac{1}{k}\sum_{p=1}^{k}\mathbb{E}_{(\bm{o}_t,\bm{a}_t)\sim\mathcal{D}^p}\left[\sum_{t=0}^{l^p}\mathcal{L}(\pi(\bm{o}_{\leq t};T^{p}),\bm{a}_{t}^{p})\right],
\end{equation}
where $\bm{s}_t\equiv\bm{o}_{\leq t}\triangleq(\bm{o}_0,\bm{o}_1,\dots,\bm{o}_t)$ is represented by the aggregated history of observations, $\mathcal{L}$ is the behavior cloning loss (\eg, the negative log-likelihood loss), and $\{\mathcal{D}^{p}:p<k\}$ is not fully available when learning $T^k$.

% To evaluate the continual learning performance, we introduce three key performance indicators: (i) average success rate, (ii) negative backward transfer (NBT), and (iii) forward transfer (FT). Detailed formulations of these metrics are provided in Appendix~\ref{appendix}.

\begin{figure*}[ht!]
    \centering
    \includegraphics[width=\linewidth]{figures/four_continual_heatmaps.pdf}
    \caption{
Comparison of the continual learning performance between the naive sequential FT and ER on the two homogeneous task streams. While naive sequential FT suffers severe performance loss on real-world data streams, ER can effectively eliminate catastrophic forgetting in both single-arm and bimanual tasks.}
    \label{fig:four_continual_heatmaps}
\end{figure*}

\section{Real-World Continual Manipulation Benchmark}\label{sec:forgetting}

Unlike simulated benchmarks, which often feature idealized dynamics and limited environmental diversity, leading to an overestimation of model robustness, real-world robotic task streams present highly non-stationary data distributions, complex physical interactions, and unpredictable environmental disturbances. To evaluate how VLA models adapt under realistic deployment conditions, this section develops a real-world continual manipulation benchmark comprising 10 diverse manipulation tasks with substantial inter-task variation. 

\paragraph{Robot Platform Setup.} As shown in Figure~\ref{fig:robot_setup}, we conducted all experiments using two PiPER-X 6-DoF robotic arms, each equipped with a parallel-jaw gripper. Additionally, four RealSense D435 are deployed to capture the visual observations: one front camera, one head camera, and two wrist-mounted cameras. More detailed hardware configurations and real-world deployment setups are provided in the Appendix.

\paragraph{Data Collection.} A leader-follower pair of robotic arms is utilized in a teleoperation framework to acquire demonstration data. We collect 500 trajectories for each single-arm task, and 300 trajectories for each bimanual task. The trajectory includes robot action records and visual sensory inputs. Visual observations are captured at 30 Hz via four RGB cameras, each stream operating at a resolution of $480 \times 640$. Finally, a 35 GB dataset is derived and stored in the LeRobot format \cite{cadene2026lerobot}.

\paragraph{Tasks Design.}
As illustrated in Figure~\ref{fig:robot_setup}, we design 5 single-arm and 5 bimanual tasks that span rigid-body manipulation (\eg, stacking and hanging), bimanual coordination, and complex deformable-object manipulation (\eg, folding clothes). This task progression introduces substantial distributional shifts in kinematics, object geometry, and contact mechanics to rigorously test skill retention. Equipped with the designed tasks, we define two distinct continual task streams. First, the \textit{homogeneous task stream} evaluates sequential learning under homogeneous control modes by training the model on either the five single-arm tasks or the five bimanual tasks independently. Second, the \textit{heterogeneous task stream} alternates between single-arm and bimanual manipulations. This design allows us to isolate and study policy degradation under structurally similar dynamics versus the interference caused by abrupt transitions in robot kinematics and control modes. Finally, we provide complete task specifications and evaluation protocols in the Appendix. 


\paragraph{Stepwise Evaluation Protocol.} Since real-world manipulation involves long-horizon execution and stochastic failures, binary success metrics are insufficient to distinguish different levels of task completion. A stepwise evaluation approach provides a more informative and reliable measure by recognizing intermediate progress, rather than focusing solely on the final outcome of success or failure. To evaluate the continual learning performance, we introduce three complementary metrics \cite{wang2024comprehensive}. (i) Denote by $c_{i,j}$ the score on the $i$-th task when evaluated using the model trained up to the $j$-th task. We report the \textbf{average score (AS)} across all tasks at the final checkpoint: $\mathrm{AS} = \frac{1}{K}\sum_{i=1}^{K} c_{i,K}.$ (ii) To quantify knowledge loss on previously learned tasks, we adopt the \textbf{backward transfer (BWT)} metric: $\mathrm{BWT}_k = \frac{1}{k-1}\sum_{j=1}^{k-1} \left(c_{j,k} - c_{j,j}\right),$ where a negative BWT indicates that performance degrades after learning subsequent tasks. The higher the value, the better. (iii) To assess whether sequential learning facilitates or hinders the acquisition of new tasks, the \textbf{forward transfer (FWT)} metric is introduced: $\mathrm{FWT}_k = \frac{1}{k-1}\sum_{j=2}^{k}\left(c_{j,j}-\bar{c}_j\right)$, where $\bar{c}_{j}$ is the single-task baseline performance. Positive $\mathrm{FWT}_i$ indicates that prior tasks facilitate learning new tasks, whereas negative $\mathrm{FWT}_i$ indicates plasticity loss.


\begin{table*}[]
\centering
\begin{tabular}{cccccccccc}
\toprule
\textbf{Type} & \textbf{Method} & $\mathcal{D}_1$ & $\mathcal{D}_2$ & $\mathcal{D}_3$ & $\mathcal{D}_4$ & $\mathcal{D}_5$ & \textbf{AS} ($\uparrow$) & \textbf{BWT} ($\uparrow$) & \textbf{FWT} ($\uparrow$) \\ \midrule
               & Baseline             & 100.0           & 97.5            & 100.0           & 52.0            & 85.0            & 86.9                          & --                         & --                      \\
Single-Arm    & Joint training  & 97.5            & 95.0            & 33.3            & 92.0            & 95.0            & 82.6                          & --                         & --                      \\
\textit{}     & Sequential FT   & 20.0            & 0.0             & 20.0            & 32.0            & 85.0            & 31.4                          &     -81.0                       &     +11.6                    \\
\textit{}     & ER              & 100.0           & 95.0            & 100.0           & 96.0            & 95.0            &  97.2                         &      +1.5                      &    +11.4                     \\ \midrule
\textit{}     & Baseline             & 90.0            & 90.0            & 96.7            & 76.7            & 86.7            & 88.0                          & --                         & --                      \\
Bimanual      & Joint training  & 80.0            & 82.5            & 93.3            & 73.3            & 86.7            &  83.2                         & --                         & --                      \\
\textit{}     & Sequential FT   & 0.0             & 5.0             & 43.3            & 50.0            & 93.3            &  38.3                         & -68.6                           &    +6.4                     \\
\textit{}     & ER              & 95.0            & 97.5            & 100.0           & 96.7            & 96.7            & 97.2                          &    +1.90                        &   +9.6                      \\ \bottomrule
\end{tabular}
\caption{Comparison of continual learning performance on real-world VLA task streams. Scores are evaluated after training on the final task and reported for all tasks.}
\label{tab:task_level_metrics}
\end{table*}


\section{Towards Robust Continual VLA Learning via Experience Replay}
Equipped with the developed benchmark, we first investigate whether the VLA models suffer from catastrophic forgetting when trained sequentially on real-world data streams. Furthermore, we investigate whether experience replay (ER) \cite{rolnick2019experience}, which interleaves historical demonstrations from a bounded buffer with the incoming data stream, can mitigate forgetting in continual VLA adaptation with real-world demonstration data. We systematically examine how key replay configurations, such as replay ratio and replay frequency, govern the overall behavior of the ER approach. In particular, we further demonstrate that selecting an appropriate action normalization strategy significantly affects the final performance of the ER approach.

\subsection{Continual Adaptation of VLA Models Under Real-World Data Streams}
\subsubsection{Model Baseline.}
We adopt $\pi_{0.5}$ \cite{black2025pi} as our base VLA model and follow its standard supervised FT pipeline. To monitor performance degradation across the continual adaptation stages, we evaluate checkpoints by rolling out the policy on each task and computing normalized scores (0-100) based on task-specific rubrics. Complete training hyperparameters, optimization schedules, and baseline configurations are deferred to the Appendix.

\subsubsection{Experience Replay Setup.}
To implement ER under practical data constraints, we maintain a replay buffer $\mathcal{B}$ with its capacity bounded by $N_\mathcal{B}=\rho_{\mathcal{B}}N_{\mathrm{ep}}$, where $\rho_{\mathcal{B}}\in(0,1]$ denotes the replay ratio and $N_{\mathrm{ep}}$ is the total number of collected episodes. To ensure balanced memory representation, this capacity is uniformly partitioned among the $K$ encountered tasks, allocating $\lfloor N_\mathcal{B}/K\rfloor$ episodes per task to prevent recent tasks from dominating the replay buffer during continual adaptation. During training, we regulate the stability-plasticity trade-off by dynamically constructing mini-batches from either the replay buffer $\mathcal{D}_{\mathrm{rep}}$ or current-task demonstrations $\mathcal{D}_{\mathrm{cur}}$. Specifically, these batches are selected according to the probability distribution $P(\mathcal{D}_{\mathrm{rep}})=f_r$ and $P(\mathcal{D}_{\mathrm{cur}})=1-f_r$, where $f_r\in[0,1]$ defines the replay frequency. 

% \subsubsection{Naive Continual Adaptation Causes Catastrophic Forgetting.}

% As illustrated in Figure~\ref{fig:continual_heatmaps} and Table~\ref{tab:task_level_metrics}, naive sequential FT incurs significant forgetting over all the tasks. For the single-arm task stream, after the model completed learning all tasks, it lost approximately 80 of its performance in the previous four tasks. Similarly, for the bimanus task stream, the model finally lost approximately 80 of its performance of the previously learned tasks. These results demonstrate that naive SFT can cause catastrophic forgetting when learning continually from the real-world data streams. Overall, due to the extremely high non-stationarity of real-world data streams, the models exhibit a much higher degree of forgetting than is observed in simulated environments \cite{liu2026pretrained}. 

\subsubsection{Naive Sequential FT Causes Catastrophic Forgetting.}
As shown in Figure~\ref{fig:four_continual_heatmaps} and Table~\ref{tab:task_level_metrics}, naive sequential FT suffers from severe catastrophic forgetting across both single-arm and bimanual task streams. 
For the single-arm stream, upon completing sequential adaptation via task $\mathcal{D}_5$, the model's AS drops sharply from $86.9$ to $31.4$, resulting in a low BWT of $-81.0$. Early tasks experience near-total performance collapse, with AS on $\mathcal{D}_1$ and $\mathcal{D}_2$ falling to $20.0$ and $0.0$, respectively. A similar failure pattern emerges in the bimanual stream, where sequential FT achieves an AS of merely $38.3$ and a BWT of $-68.6$, losing the vast majority of previously learned capabilities. These results demonstrate that standard sequential FT fails under deployment-realistic streams. Crucially, due to the pronounced non-stationarity of real-world physical data, VLA models exhibit a higher degree of forgetting than previously reported in simulated benchmarks \cite{liu2026pretrained}.

\subsection{Well-Configured ER Effectively Eliminates Catastrophic Forgetting}

\subsubsection{Small Replay Budgets Preserve Previous Skills and Enable Transfer.} 

ER effectively restores stability in continual learning, even under a minimal replay budget. As shown in Table~\ref{tab:task_level_metrics}, equipping sequential FT with ER achieves an AS of $97.2$ across both single-arm and bimanual streams, substantially drastically reducing forgetting to minimal degradation (BWT of $+1.5$ and $+1.9$, respectively). Remarkably, well-configured ER consistently outperforms joint multi-task training under equivalent computational budgets, which achieves an AS of only $82.6$ on the single-arm stream and $83.2$ on the bimanual stream. This superiority stems from the fact that joint training on heterogeneous physical tasks suffers from optimization conflicts and gradient interference when all skills are optimized simultaneously. In contrast, sequential learning with ER enables staged representation learning while maintaining historical stability through replay.


\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{figures/er_sensitivity.pdf}
    \caption{Sensitivity analysis of ER configurations. Increasing buffer capacity enhances retention, while replay frequency presents a stability–plasticity trade-off between insufficient (forgetting) and excessive (over-regularization) replay.}
    \label{fig:er_sensitivity}
\end{figure}

% \subsubsection{Replay Frequency Balances Stability and Plasticity.}
% To study the impact of ER configurations on final performance, we run a hyperparameter sweep over the buffer ratio $\{0.002,0.02,0.2\}$ and the replay frequency $\{0.05,0.1,0.2,0.5\}$. The performance of ER depends on balancing retention and adaptation. Figure~\ref{fig:er_sensitivity} shows that properly configured replay preserves performance across the task sequence, while replay frequency introduces a clear stability--plasticity trade-off. Insufficient replay ($f_r=0.05$) weakens retention, whereas excessive replay ($f_r=0.5$) limits adaptation to new tasks. Generally, the optimal setting around $f_r=0.2$ effectively preserves prior skills without sacrificing new-task learning.

\subsubsection{Replay Frequency Balances Stability and Plasticity.}
We evaluate ER sensitivity across buffer ratios $\rho_{\mathcal{B}} \in \{0.002, 0.02, 0.2\}$ and replay frequencies $f_r \in \{0.05, 0.1, 0.2, 0.5\}$. As shown in Figure~\ref{fig:er_sensitivity}, increasing buffer capacity improves retention, increasing final average BWT from $-8.95$ ($\rho_{\mathcal{B}} = 0.002$) to $+0.25$ ($\rho_{\mathcal{B}} = 0.02$) and $+1.50$ ($\rho_{\mathcal{B}} = 0.2$), proving that a modest buffer ($\rho_{\mathcal{B}} = 0.02$) is already highly effective. Conversely, replay frequency $f_r$ governs a distinct stability--plasticity trade-off. Low frequency ($f_r = 0.05$) leads to high forgetting ($\text{BWT} = -21.1$), whereas increasing $f_r$ to $0.1$ and $0.2$ progressively raise BWT to $-8.75$ and $+1.50$, respectively. Although aggressive replay ($f_r = 0.5$) achieves the highest BWT ($+8.68$), it over-regularizes the policy and impairs adaptation to new tasks. Consequently, $f_r = 0.2$ provides the optimal balance between historical skill retention and new-task plasticity.


\begin{figure}[t!]
    \centering
    % \includegraphics[width=\linewidth]{figures/HyperparameterSensitivity.pdf}
    \includegraphics[width=\linewidth]{figures/ans_comparison.pdf}
    \caption{Comparison of the continual learning performance across three action normalization strategies. Here, \textbf{ANS \Rmnum{2}} achieves the best performance in both single-arm and bimanual task streams, highlighting the importance of maintaining action normalization consistency in the continual learning process.}
    \label{fig:ans}
\end{figure}

\subsection{Action Normalization Consistency Is Critical for Continual Adaptation}

Continual VLA learning requires a consistent action coordinate system throughout continual adaptation. Since future task data is unavailable, normalization statistics must be determined before training. In this paper, we design and test three distinct action normalization strategies (ANS). Specifically, \textbf{ANS \Rmnum{1}}: The policy is trained and tested on each task using its local, task-specific action statistics. \textbf{ANS \Rmnum{2}}: The normalization statistics of the first task are frozen and applied to the entire task stream for both training and testing. \textbf{ANS \Rmnum{3}}: The model is trained sequentially using each task's individual normalization statistics, yet the normalization statistics of the first task are utilized for all the testing.

% \begin{table}[ht!]
% \begin{tabular}{llcccccc}
% \toprule
% \textbf{Type} & \textbf{Method} & $\mathcal{D}_1$ & $\mathcal{D}_2$ & $\mathcal{D}_3$ & $\mathcal{D}_4$ & $\mathcal{D}_5$ & \textbf{Avg.($\uparrow$)} \\ \midrule
%               & ANS \Rmnum{1}   & 95              & 40              & 0               & 20              & 70              & 45                        \\
% Single-Arm    & ANS \Rmnum{2}   & 100             & 95              & 100             & 96              & 95              & 97.2                      \\
% \textit{}     & ANS \Rmnum{3}   & 95              & 15              & 0               & 20              & 65              & 39                        \\ \hline
% \textit{}     & ANS \Rmnum{1}   & 86.7            & 82.5            & 28.3            & 58.3            & 9               & 52.96                     \\
% Bimanual      & ANS \Rmnum{2}   & 95              & 97.5            & 100             & 96.7            & 96.7            & 97.2                      \\
% \textit{}     & ANS \Rmnum{3}   & 86.7            & 0               & 0               & 0               & 0               & 17.34                     \\ \hline
% \end{tabular}
% \end{table}

We find that a fixed normalization space can support effective continual learning when it provides sufficient action coverage. Using the first-task statistics (\textit{stack bowls} for single-arm and \textit{cook bread} for bimanual sequences), models achieve stable optimization and strong performance across subsequent tasks. In contrast, allowing normalization statistics to vary across tasks disrupts cross-task alignment, preventing reliable knowledge transfer even when task-specific behaviors are successfully learned. These results indicate that maintaining a shared action space is more important than adapting normalization independently for each task.

\section{Continual Adaptation on Heterogeneous Task Stream}

Building upon the insights gained from evaluations of homogeneous task streams, which established effective ER configurations and the critical role of action normalization strategy, we scale our investigation to a significantly more challenging deployment scenario. In this section, we evaluate continual adaptation on a long-horizon, heterogeneous task stream comprising all ten manipulation tasks, executed in alternating order. Unlike homogeneous streams that preserve uniform robot kinematics, this heterogeneous protocol constantly interleaves single-arm and bimanual tasks. This setup introduces severe non-stationarity by forcing a single policy to adapt to a sequence characterized by abrupt, recurring transitions in control dimensionality, kinematic configurations, and physical contact dynamics. By testing the model on this complex task stream, we investigate whether our ER framework and action normalization strategies can mitigate cross-task interference and prevent policy collapse in the face of diverse physical-manipulation demands.

\begin{figure}[ht!]
    \centering
    \includegraphics[width=\linewidth]{figures/heterogeneous_matrix.pdf}
    \caption{The continual learning performance on the heterogeneous task stream. Our method achieves stable continual learning across the long-horizon task sequence, with consistent retention and adaptation throughout all checkpoints.}
    \label{fig:heterogeneous_matrix}
\end{figure}

\begin{figure}[ht!]
    \centering
    % \includegraphics[width=\linewidth]{figures/HyperparameterSensitivity.pdf}
    \includegraphics[width=\linewidth]{figures/hetero_bwt_fwt.pdf}
    \caption{Trace of the BWT and FWT metrics across the heterogeneous task stream. A uniform replay frequency across all tasks degrades performance in bimanual tasks, whereas an asymmetric replay schedule effectively eliminates forgetting.}
    \label{fig:hetero_nbt_ft}
\end{figure}

% \paragraph{Training Configuration.} We train the policy sequentially on the heterogeneous task stream for $4,000$ steps per task. The ER framework is configured using a replay ratio of $0.2$ and a replay frequency of $0.2$. For action normalization, we adopt the \textbf{ANS \Rmnum{2}}. Since the heterogeneous sequence initiates with a single-arm task, the normalization parameters calculated from the active arm are replicated to the left arm to establish a consistent initialization baseline across both arms before transitioning to bimanual tasks. All other training parameters, architectures, and optimization hyperparameters remain identical to the previously described protocols.
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/snapshot.pdf}
    % \includegraphics[width=\linewidth,height=8cm]{example-image-a}
    \caption{Qualitative rollout snapshots evaluated after completing the full 10-task heterogeneous continual learning stream. Representative keyframes showcasing physical robot execution on selected single-arm and bimanual tasks. The final adapted policy demonstrates robust execution and skill retention across diverse manipulation primitives after sequential training across all 10 tasks, without suffering from catastrophic forgetting or action collapse.}
    \label{fig:hetero_demos}
\end{figure*}

\paragraph{Overall Continual Performance.} We first evaluate the overall efficacy of the adapted policy across the entire 10-task heterogeneous stream. As illustrated in the performance matrix (Figure~\ref{fig:heterogeneous_matrix}) and the rollout snapshots (Figure~\ref{fig:hetero_demos}), the policy successfully acquires new manipulation skills sequentially while retaining previously learned behaviors. Rather than suffering from catastrophic forgetting or action mode collapse, the agent maintains robust execution across both single-arm and bimanual tasks throughout the adaptation process. To quantitatively analyze the adaptation dynamics, Figure~\ref{fig:hetero_nbt_ft} presents the task-by-task BWT and FWT. The bar components show the FWT for each task, maintaining a remarkably high average of $+8.7$ by the final stage. Simultaneously, the line plot traces the BWT across the task sequence, yielding an average BWT of $-2.7$. This dual-metric analysis reveals that our ER-based strategy effectively balances stability and plasticity, minimizing backward interference while facilitating positive forward transfer even across abrupt kinematic transitions.

\paragraph{Asymmetric Replay Schedule for Kinematic Transitions.}
A key empirical insight from our heterogeneous stream evaluation is that applying a uniform replay frequency across all tasks yields suboptimal stability. Specifically, when employing the default homogeneous configuration ($f_r = 0.2$), the policy experiences severe performance degradation on previously learned bimanual tasks when adapting to subsequent single-arm tasks. This heightened vulnerability arises because bimanual manipulation inherently requires higher-dimensional spatial coordination and exhibits complex control dynamics, making its task representations particularly fragile to parameter overwriting. Furthermore, when the model transitions to single-arm tasks, optimization focuses exclusively on a single arm, generating gradient updates that actively suppress and unlearn the action outputs associated with the inactive arm. To counter this cross-kinematic interference, we introduce an asymmetric replay schedule. Specifically, we increase the overall replay frequency to $f_r=0.3$ and bias the replay buffer sampling toward bimanual experiences at a $2:1$ ratio relative to single-arm experiences. This design ensures that the model anchors the complex dual-arm coordination patterns with sufficient frequency, while still retaining adequate plasticity to adapt to subsequent single-arm tasks.

\section{Conclusion}
In this work, we establish a real-world continual manipulation benchmark to systematically evaluate VLA models' adaptation under physical deployment constraints. Through extensive experiments on heterogeneous manipulation tasks, we demonstrate that naive sequential FT suffers from severe catastrophic forgetting due to the high non-stationarity of real-world physical data. We show that well-configured ER effectively eliminates skill degradation while enabling positive forward transfer. Surprisingly, our results reveal that continual learning-based training can outperform joint multi-task training under equivalent computational budgets. 

Despite these insights, our study presents several limitations that open promising avenues for future research. First, our investigation focuses primarily on replay-based adaptation within a fixed physical platform setup. Extending continual adaptation mechanisms to cross-embodiment setups, broader task distributions, and open-ended long-horizon scenarios remains an unaddressed challenge. Second, while ER effectively maintains policy stability, storing historical demonstration data may increase memory demands over prolonged, lifelong deployment. Future work could explore parameter-efficient modular adapters, exemplar-free architectures, and active memory management. This paper is expected to inspire more subsequent research toward building scalable, robust, and truly lifelong embodied agents. 
